DynAMO: Multi-agent reinforcement learning for dynamic anticipatory mesh optimization with applications to hyperbolic conservation laws

We introduce DynAMO, a reinforcement learning paradigm for Dynamic Anticipatory Mesh Optimization. Adaptive mesh refinement is an effective tool for optimizing computational cost and solution accuracy in numerical methods for partial differential equations. However, traditional adaptive mesh refinement approaches for time-dependent problems typically rely only on instantaneous error indicators to guide adaptivity. As a result, standard strategies often require frequent remeshing to maintain accuracy. In the DynAMO approach, multi-agent reinforcement learning is used to discover new local refinement policies that can anticipate and respond to future solution states by producing meshes that deliver more accurate solutions for longer time intervals. By applying DynAMO to discontinuous Galerkin methods for the linear advection and compressible Euler equations in two dimensions, we demonstrate that this new mesh refinement paradigm can outperform conventional threshold-based strategies while also generalizing to different mesh sizes, remeshing and simulation times, and initial conditions.

==> outline.tex <==
\setcounter{section}{-1}\section{Paper outline}
\begin{adjustwidth}{0.05\linewidth}{0.05\linewidth}
\nointerlineskip\leavevmode
Work in progress, feel free to add/modify - TD



\subsection{Introduction}
\paragraph{Related works}
\paragraph{Outline}
\subsection{Preliminaries}
\paragraph{Hyperbolic conservation laws}
\begin{enumerate}
    \item Introduce general nonlinear conservation law
    \item Show advection example
    \item Show Euler example
    \item Introduce flux Jacobian formulation
\end{enumerate}
\paragraph{Finite element methods}
\begin{enumerate}
    \item Broadly describe FEM, mesh and solution approximation
    \item Introduce DG for hyperbolic conservation laws, brief description of weak formulation, interface flux + Riemann solver
\end{enumerate}
\paragraph{Adaptive mesh refinement}
\begin{enumerate}
    \item Introduce $h$ and $p$ refinement (gloss over other methods, $hp$, $r$)
    \item Error estimators (general description, wait until Implementation section to go into $p-1$/SolJump)
    \item More in-depth description of drawbacks in current methods for hyperbolic PDEs (longer regrid times, direction of information propagation) 
\end{enumerate}
\paragraph{Reinforcement learning}
\begin{enumerate}
    \item Description of Markov process
    \item General overview of observation/action/transition/reward pipeline (not anything AMR specific)
\end{enumerate}

\subsection{Methodology}
 First give overarching description of the approach + goals (agents, regrids, etc.)
\paragraph{Dynamic mesh optimization as a decentralized partially observable Markov decision process}
\begin{enumerate}
    \item Agent: Describe $p$-ref vs. $h$-ref agents, give benefits of local/multi-agent approach, mention here that we look at one-level refinement but give brief overview on how we could extend to more levels (cite AAMAS paper)
    \item Observation space: Start with what properties we're interested in (transformation invariance, solution/error normalization, local domain of influence, temporal independence). Describe local observation setup. Introduce normalized error observation (abstract description of error estimate, leave until Implementation section to give in-depth detail of the error estimators for given problems). Introduce flux transport rate (describe its properties and how they link to the goals, show connections between advection and Euler, describe what problems we avoid with this formulation). Primitive + conserved variable observation.  
    \item Action space: Rewrite for consistency with current setup (increment base action space). Describe $h$-ref/$p$-ref actions. Mention eval time changes 
    \item Transition: Looks good
    \item Reward: Rewrite for consistency with current setup (increment base action space, zero reward cases, max error over regrid time), more detail on why we chose this formulation and what problems we avoid that a raw error would run into
\end{enumerate}
\paragraph{Fully-decentralized independent Proximal Policy Optimization}
\subsection{Implementation}
\paragraph{Solver}
\begin{enumerate}
    \item Introduce MFEM
    \item Solver paramters (order, basis, meshes, limiters)
    \item Error estimators
    \item Boundary conditions (periodicity, periodized ICs, description of extension to non-periodic BCs)
\end{enumerate}
\paragraph{Reinforcement learning framework}
\begin{enumerate}
    \item RLLib
    \item Environment parameters (observation neighborhood size and its connection to regrid time, observed fields, reward field)
    \item Training/eval overview
\end{enumerate}
\subsection{Results}
\paragraph{Advection with $p$-refinement}
\paragraph{Advection with $h$-refinement}
\paragraph{Euler with $p$-refinement}
\paragraph{Euler with $h$-refinement}
\begin{enumerate}
    \item Train policy on general 2D Riemann problems, apply to RP, Sod, triple point
    \item Show example AMR meshes figures and Pareto plots for the 6 RP cases from \citet{Liska2003}
    \item Show efficiency across 100 general RP 
    \item Show efficiency across 100 general RP with longer simulation time
    \item Show efficiency across 100 general RP with larger regrid time
    \item Show efficiency across 100 general RP with larger mesh
    \item Show Pareto plot + mesh for 2D Sod case 
    \item Show Pareto plot + mesh for triple point case
\end{enumerate}

\end{adjustwidth}

==> scratch.tex <==

% \begin{table}[htbp!]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%     Method & Efficiency (In-distribution) &  Efficiency (Longer simulation time) \\ 
%     \midrule
%     Threshold ($\theta = 10^{0}$)\hphantom{1} &  0.008 (0.018) & 0.037 (0.046) \\
%     Threshold ($\theta = 10^{-1}$) & 0.215 (0.083) &  \textbf{0.226 (0.096)} \\
%     Threshold ($\theta = 10^{-2}$) & \textbf{0.251 (0.056)} &  0.202 (0.065) \\
%     Threshold ($\theta = 10^{-3}$) & 0.180 (0.031) &  0.084 (0.022) \\
%     Threshold ($\theta = 10^{-4}$) & 0.162 (0.027) &  0.075 (0.021) \\
%     Threshold ($\theta = 10^{-5}$) & 0.157 (0.027) &  0.073 (0.021) \\
%     Threshold ($\theta = 10^{-6}$) & 0.157 (0.027) &  0.073 (0.021) \\
%     \midrule
%     DYNAMO & \textbf{0.486 (0.073)} & \textbf{0.423 (0.113)} \\
%     DYNAMO/Optimal $\theta$ & \textcolor{green!70!black}{+93.6\%}  & \textcolor{green!70!black}{+87.2\%} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:euler_href_longersimtime} Comparison of the mean efficiency for $h$-refinement on the Euler equations with DYNAMO and the threshold policy for the two-dimensional Riemann problem over 100 \textit{out-of-distribution} runs using uniform random initial conditions with longer simulation time. Standard deviation shown in parentheses. In-distribution results from \cref{tab:euler_href_indistribution} shown for comparison.}
% \end{table}

% \begin{table}[htbp!]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%     Method & Efficiency (In-distribution) &  Efficiency (Longer regrid time) \\ 
%     \midrule
%     Threshold ($\theta = 10^{0}$)\hphantom{1} &  0.008 (0.018) & 0.038 (0.048) \\
%     Threshold ($\theta = 10^{-1}$) & 0.215 (0.083) & \textbf{0.243 (0.099)} \\
%     Threshold ($\theta = 10^{-2}$) & \textbf{0.251 (0.056)} & 0.235 (0.065) \\
%     Threshold ($\theta = 10^{-3}$) & 0.180 (0.031) & 0.147 (0.036) \\
%     Threshold ($\theta = 10^{-4}$) & 0.162 (0.027) & 0.145 (0.035) \\
%     Threshold ($\theta = 10^{-5}$) & 0.157 (0.027) & 0.145 (0.035) \\
%     Threshold ($\theta = 10^{-6}$) & 0.157 (0.027) & 0.145 (0.035) \\
%     \midrule
%     DYNAMO & \textbf{0.486 (0.073)} & \textbf{0.461 (0.088)} \\
%     DYNAMO/Optimal $\theta$ & \textcolor{green!70!black}{+93.6\%} & \textcolor{green!70!black}{+89.7\%} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:euler_href_longerregridtime} Comparison of the mean efficiency for $h$-refinement on the Euler equations with DYNAMO and the threshold policy for the two-dimensional Riemann problem over 100 \textit{out-of-distribution} runs using uniform random initial conditions with longer regrid time. Standard deviation shown in parentheses. In-distribution results from \cref{tab:euler_href_indistribution} shown for comparison.}
% \end{table}

% \begin{table}[htbp!]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%     Method & Efficiency (In-distribution) &  Efficiency (Finer mesh) \\ 
%     \midrule
%     Threshold ($\theta = 10^{0}$)\hphantom{1} &  0.008 (0.018) & 0.047 (0.063) \\
%     Threshold ($\theta = 10^{-1}$) & 0.215 (0.083) & 0.280 (0.102) \\
%     Threshold ($\theta = 10^{-2}$) & \textbf{0.251 (0.056)} & \textbf{0.328 (0.082)} \\
%     Threshold ($\theta = 10^{-3}$) & 0.180 (0.031) & 0.245 (0.051) \\
%     Threshold ($\theta = 10^{-4}$) & 0.162 (0.027) & 0.212 (0.041) \\
%     Threshold ($\theta = 10^{-5}$) & 0.157 (0.027) & 0.193 (0.035) \\
%     Threshold ($\theta = 10^{-6}$) & 0.157 (0.027) & 0.180 (0.030) \\
%     \midrule
%     DYNAMO & \textbf{0.486 (0.073)} & \textbf{0.545 (0.069)} \\
%     DYNAMO/Optimal $\theta$ & \textcolor{green!70!black}{+93.6\%} & \textcolor{green!70!black}{+66.2\%} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:euler_href_finermesh} Comparison of the mean efficiency for $h$-refinement on the Euler equations with DYNAMO and the threshold policy for the two-dimensional Riemann problem over 100 \textit{out-of-distribution} runs using uniform random initial conditions with finer mesh resolution. Standard deviation shown in parentheses. In-distribution results from \cref{tab:euler_href_indistribution} shown for comparison.}
% \end{table}

% \begin{table}[htbp!]
%     \centering
%     \begin{tabular}{cc}
%     \toprule
%     Method &  Efficiency \\ 
%     \midrule
%     Threshold ($\theta = 10^{-4}$) & 0.389 (0.102) \\
%     Threshold ($\theta = 10^{-5}$) & 0.473 (0.106) \\
%     Threshold ($\theta = 10^{-6}$) & \textbf{0.478 (0.096)} \\
%     Threshold ($\theta = 10^{-7}$) & 0.432 (0.101) \\
%     Threshold ($\theta = 10^{-8}$) & 0.351 (0.109) \\
%     \midrule
%     DYNAMO & \textbf{-(-)} \\
%     DYNAMO/Optimal $\theta$ & \textcolor{green!70!black}{+0\%} \\
%     \bottomrule
%     \end{tabular}
%     \caption{\label{tab:advection_href_indistribution} Comparison of the mean efficiency for $h$-refinement on the advection equation with DYNAMO and the threshold policy for the advecting Gaussian bump over 100 \textit{in-distribution} runs using uniform random initial conditions. Standard deviation shown in parentheses.}
% \end{table}


Discussion of the progress of test problems, and the motivation for the introduction of each one, outlining how the first problems are more proof of principle, and the following problem introduce more physics content and complexity to see if the method holds up in a more realistic setting with more physics content.


In distribution -  \\
Out distribution - AAMAS paper for advection.
longer simulation, larger meshes, different functions (e.g. ring function), number of features (e.g. multiple bumps)


% \begin{table}[htb]
%     \centering
%     \caption{Use \texttt{P-1} error estimator for all p-refinement policies, and \texttt{SolJump} for h-refinement}
%     \begin{tabular}{ccccc}
%         \toprule
%         problem & ref mode & who trains RL & pareto baseline done? & 100 random IC baselines done? \\
%         \midrule
%         advection & p & Ketan & yes & yes \\
%         advection & h & Tarik & yes & yes \\
%         advection reward mod & p & Dohyun \\
%         advection reward mod & h & Dohyun & yes\\        
%         vortex & p & Ketan & yes & yes \\
%         vortex & h & \\
%         pulse & p & Ketan & yes & yes \\
%         pulse & h & \\
%         Sod & h & Tarik & yes \\
%         Riemann & h & Tarik \\
%         \bottomrule
%     \end{tabular}
    
%     \label{tab:my_label}
% \end{table}

%Euler
% General training - 
% Out of distribution tests (smooth): (Ketan)
% 
% * Euler vortex
% * Kelvin Helmholtz
% * 
% h-refinement test cases:
% * Sod shock tube (Tarik, Bob)
%   * Randomized 2-state shock tube conditions training set
%   * Standard "Sod" conditions for test
%   * Error from exact solution
%   * current roadblocks - robustness? 
% * Euler vortex (Bob)
%   * 
% * Kelvin Helmholtz (???)

% Figures
% * pareto plot on cost/err axes, comparing estimate/threshold to policy
% * comparison of error vs time, show comparison of regrid periods between threshold and policy to get comparable rates of error growth

% [ ] Capability to discard runs that crash - needs rllib version that's newer than ours - Jiachen and Ketan
% [ ] Seeing if we can upgrade rllib without changing other library versions or having other issues - Jiachen and Ketan
% [ ] Jiachen volunteers to run baselines for the cases (thresholding method)
% [ ] Bob will supply Jiachen with conditions for Sod shock tube to start (config file if it exists, or create a new one)
% [ ] multi-level refinement for h to have it in hand in case it is required of us (Jiachen)

% Euler vortex, Kelvin Helmholtz, Rayleigh Taylor, Taylor vortices
% 


% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/advection_href_pareto_contour_exact.eps}
%     \caption{Advection $p$-refinement}
%     % \label{fig:}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/advection_href_pareto_contour_exact.eps}
%     \caption{Advection $h$-refinement}
%     \label{}
%     \end{subfigure}
% \caption{Advection h-refinement (left).}
% \label{fig:pareto_advection}
% \end{figure}

% \begin{figure}[t]
% \centering
%     % tstep 0.5 tfinal 3
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/advection_pref_pareto_contour_zz_tstep0p5_tfinal3.png}
%     \caption{Advection $p$-refinement}
%     % \label{fig:}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/advection_href_pareto_contour_zz.png}
%     \caption{Advection $h$-refinement}
%     \label{}
%     \end{subfigure}
% \caption{Advection}
% \label{fig:pareto_advection}
% \end{figure}


% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep2_tfinal8/vortex_pareto_contour_pm1_est3_idx0.png}
%     \caption{Vortex comp 1}
%     % \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep2_tfinal8/vortex_pareto_contour_pm1_est3_idx1.png}
%     \caption{Vortex comp 2}
%     \label{}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep2_tfinal8/vortex_pareto_contour_pm1_est3_idx2.png}
%     \caption{Vortex comp 3}
%     \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep2_tfinal8/vortex_pareto_contour_pm1_est3_idx3.png}
%     \caption{Vortex comp 4}
%     \label{fig:}
%     \end{subfigure}
% \caption{Euler vortex with p-refinement. tstep2 tfinal8}
% \label{fig:pareto_vortex_p_tstep2_tfinal8}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep8_tfinal40/vortex_pareto_contour_pm1_est3_idx0.png}
%     \caption{Vortex comp 1}
%     % \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep8_tfinal40/vortex_pareto_contour_pm1_est3_idx1.png}
%     \caption{Vortex comp 2}
%     \label{}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep8_tfinal40/vortex_pareto_contour_pm1_est3_idx2.png}
%     \caption{Vortex comp 3}
%     \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/vortex_pref_tstep8_tfinal40/vortex_pareto_contour_pm1_est3_idx3.png}
%     \caption{Vortex comp 4}
%     \label{fig:}
%     \end{subfigure}
% \caption{Euler vortex with p-refinement. tstep8 tfinal40}
% \label{fig:pareto_vortex_p_tstep8_tfinal40}
% \end{figure}

% % Best top-p params: 0.1, 0.4
% % Best ST param: 5e-7
% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/pulse_pareto_contour_pm1_est3_idx0.png}
%     \caption{pulse comp 1}
%     % \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/pulse_pareto_contour_pm1_est3_idx1.png}
%     \caption{pulse comp 2}
%     \label{}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/pulse_pareto_contour_pm1_est3_idx2.png}
%     \caption{pulse comp 3}
%     \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/pulse_pareto_contour_pm1_est3_idx3.png}
%     \caption{pulse comp 4}
%     \label{fig:}
%     \end{subfigure}
% \caption{Euler pulse with p-refinement}
% \label{fig:pareto_pulse_p}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/sod_pareto_contour_soljump_est2_idx1.png}
%     \caption{Sod comp 1}
%     % \label{fig:}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[t]{0.24\linewidth}
%     \includegraphics[width=1.0\linewidth]{fig_pareto/sod_pareto_contour_soljump_est2_idx2.png}
%     \caption{Sod comp 2}
%     \label{}
%     \end{subfigure}
% \caption{Euler Sod with h-refinement}
% \label{fig:pareto_sod_h}
% \end{figure}


% The best parameters for SingleThreshold and Top-p from the Pareto sweep were used for this 100 IC test.
% Parameters for ST
% advection p-ref: 5e-5
% advection h-ref: 5e-5
% pulse p-ref: 5e-7
% vortex p-ref: 2e-3

% Parameters for Top-p
% advection p-ref: low 0.1 high 0.2
% advection h-ref: low 0.1 high 0.1
% pulse p-ref: 0.1, 0.4
% vortex p-ref: 0.1, 0.3
% \begin{table*}[t]
%     \centering
%     \caption{Mean and standard error of efficiency of DynAMO versus heuristic policies, over 100 runs with uniform random ICs.}
%     \begin{tabular}{crrrrrr}
%     \toprule
%     Method & Advection (p) & Advection (h) & Pulse & Vortex & Sod & Riemann \\ 
%     \midrule
%     Single Threshold & 0.883 (0.013) & 0.898 (0.013) & 0.444 (0.010) & 0.864 (0.003) \\
%     Top-$p$ & 0.823 (0.012) & 0.839 (0.012) & 0.373 (0.009) & 0.742 (0.003) \\ 
%     \midrule
%     DynAMO \\ 
%     \bottomrule
%     \end{tabular}
%     \label{tab:efficiency_in_distribution}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \caption{Mean and standard error of efficiency of DynAMO versus heuristic policies, over 100 runs on out-of-distribution problems with uniform random ICs.}
%     \begin{tabular}{crrrrrrrrrrrrr}
%     \toprule
%     Method & Advection (p) & Advection (h) & Pulse & Vortex & Sod & Riemann \\
%     \midrule
%     Single Threshold &  \\
%     Top-$p$ &  \\ 
%     \midrule
%     DynAMO \\ 
%     \bottomrule
%     \end{tabular}
%     \label{tab:efficiency_generalization}
% \end{table*}



% using a graph neural network. Another approach using reinforcement learning for AMR was proposed by Foucart et al.~\cite{foucart2023deep}. One of the key differences is that the authors formulated AMR as a partially observed Markov decision process where an agent in each element can observe only the neighboring elements' error indicators. Also, the former approach used the exact error as an error estimator, but the latter only used local jump as an error indicator.

% In \cite{yang2021reinforcement}, the authors formulate AMR as a Markov decision process with \emph{variable}-size state and action spaces.
% The authors then propose novel policy architectures to support these non-standard variable-size spaces.
% Due to the complexity of training on large meshes, the training approach in \cite{yang2021reinforcement} relie
% Another novelty in \cite{yang2021reinforcement} is that the authors do not rely on existing error estimators from the finite element literature.
% Instead, they replace the \textsc{estimate} and \textsc{mark} steps in~\eqref{} with an element-wise decision based on a direct view of the localized solution about each element.

% This class of methods approximates a mesh density function \cite{tan2003proper} in the physical domain which can then be used to generate computational meshes with downstream mesh generators \citep{dobrzynski2008anisotropic,budd2009moving}. 

% Other approaches also show promising results, including but not limited to selecting the optimal D\"orfler marking index \cite{gillette2022learning}, finding the hyper-parameters for the extension operator \cite{zhang2023extension}, and measuring the mesh quality \cite{zhang2023mqenet}.


% This class of approaches continues to be actively developed \cite{}.
% Other approaches also show promising results, including but not limited to selecting the optimal D\"orfler marking index \cite{gillette2022learning}, finding the hyper-parameters for the extension operator \cite{zhang2023extension}, and measuring the mesh quality \cite{zhang2023mqenet}.

% TODO (LATER)

% \smallskip
% The ice hockey star Wayne Gretzky famously said, ``I skate to where the puck is going, not where it has been.''
% Likewise, the aim of DynAMO is to refine the mesh where the error will propagate, not where it is presently.

% \subsection{Related work} % (fold)
% \label{sub:literature_review}

% Adaptive mesh refinement (AMR) promises cost-effective numerical simulations by allowing resources to be applied only near the ``areas of interest''. This approach is now widely used because of theoretical advances \cite{zienkiewicz1992superconvergent1,zienkiewicz1992superconvergent2, carstensen2014axioms} and software supports \cite{mfem, fenicsx, fluent, openfoam}. However, there are many open questions and parameters to be tuned in the AMR procedures. This and recent success of machine learning techniques drew attention of many computational scientists to combine machine learning (ML) and AMR. To the best of authors' knowledge, the earliest attempt to combine ML and AMR can be traced back to early 1990s \cite{dyck1992determining}. Since then, attention has grown significantly \cite{bao2019data, bohn2021recurrent, chen2020output, pfaff2020learning, zhang2020meshingnet, huang2021machine, paszynski2021deep, sluzalec2022quasi, chen2021output, chakraborty2021multigoaloriented, roth2022neural, sprave2021evaluating, patel2021smart, yang2021reinforcement, antonietti2022machine, antonietti2022refinement}.
% [Taken from \cite{gillette2022learning}. Needs to be refashioned for this work]

% Machine learning for adaptive mesh refinement (AMR) was first studied in the early 1990s \cite{dyck1992determining}, with only a small number of subsequent contributions \cite{chedid1996automatic,manevitz2005neural} appearing in the literature until a few years ago.
% Since then, attention has grown significantly \cite{bao2019data,bohn2021recurrent,chen2020output,pfaff2020learning,zhang2020meshingnet,huang2021machine,paszynski2021deep,chen2021output,chakraborty2021multigoaloriented,roth2022neural,sprave2021evaluating,patel2021smart,yang2021reinforcement,antonietti2022machine,antonietti2022refinement}.
% To date, machine learning has been used to design goal-oriented AMR strategies \cite{chen2020output,chen2021output,chakraborty2021multigoaloriented,roth2022neural}, $hp$-refinement strategies \cite{paszynski2021deep,sluzalec2022quasi}, and refinement strategies for polygonal discretizations \cite{antonietti2022machine,antonietti2022refinement}.
% , as well as control other aspects of the discretion\ldots and flux-limiters \cite{ray2018artificial,beck2020neural,nguyen2021machine}.

% One of the actively researched approaches is mesh density function-based mesh adaptation \cite{dyck1992determining, chedid1996automatic}. This class of approaches approximates a mesh density function \cite{tan2003proper} in the physical domain.
% % The earliest data-driven approaches to AMR involved learning a mesh density function \cite{dyck1992determining,chedid1996automatic,tan2003proper} or ``areas of interest'' in the physical domain for refinement \cite{manevitz2005neural}.
% Then the mesh density function can be used to generate computational meshes using downstream mesh generators \cite{dobrzynski2008anisotropic} or some form of mesh transport \cite{budd2009moving}.
% This class of approaches continues to be actively developed \cite{pfaff2020learning,huang2021machine,zhang2020meshingnet,song2022m2n,chan2022locally}.
% Other approaches also show promising results, including but not limited to selecting the optimal D\"orfler marking index \cite{gillette2022learning}, finding the hyper-parameters for the extension operator \cite{zhang2023extension}, and measuring the mesh quality \cite{zhang2023mqenet}.

% We note that density-based AMR typically relies on a down-stream mesh generator (see, e.g., \cite{dobrzynski2008anisotropic}) or some form of mesh transport (see, e.g., \cite{budd2009moving}).
% Among other reasons, this makes density-based AMR fundamentally different from marked element AMR, which is the paradigm considered in this work.

% [rephrase] The first instance of machine learning for marked element AMR that we are aware of is \cite{bohn2021recurrent}.
% In \cite{bohn2021recurrent}, it is shown that error estimation (cf. \textsc{estimate}) and element marking (cf.~\textsc{mark}) for an elliptic partial differential equation (PDE) can be represented by a recurrent neural network.

% In Yang et al.~\cite{yang2021reinforcement}, on the other hand, AMR was first understood as a sequential decision-making problem. They observed both scaled local errors and handled \emph{variable}-size state and action spaces using a graph neural network. Another approach using reinforcement learning for AMR was proposed by Foucart et al.~\cite{foucart2023deep}. One of the key differences is that the authors formulated AMR as a partially observed Markov decision process where an agent in each element can observe only the neighboring elements' error indicators. Also, the former approach used the exact error as an error estimator, but the latter only used local jump as an error indicator.

% In \cite{yang2021reinforcement}, the authors formulate AMR as a Markov decision process with \emph{variable}-size state and action spaces.
% The authors then propose novel policy architectures to support these non-standard variable-size spaces.
% Due to the complexity of training on large meshes, the training approach in \cite{yang2021reinforcement} relie
% Another novelty in \cite{yang2021reinforcement} is that the authors do not rely on existing error estimators from the finite element literature.
% Instead, they replace the \textsc{estimate} and \textsc{mark} steps in~\eqref{} with an element-wise decision based on a direct view of the localized solution about each element.

% Although we also characterize AMR as a sequential decision-making problem, our means are different from \cite{yang2021reinforcement} in numerous ways: for example, (1) we formulate AMR as an MDP with \emph{fixed}-size state and action spaces; (2) we rely on policy architectures commonly used in reinforcement learning; and (3) our approach requires the user to provide an \emph{a posteriori} error estimator/indicator \cite{ainsworth2000aposteriori}.
% Our contribution, as well as \cite{yang2021reinforcement}, aligns with a recent trend in reinforcement learning to improve adaptive algorithms in scientific computing; for example, adaptive time-stepping for numerical integration \cite{dellnitz2021efficient} and adaptive coarsening for algebraic multi-grid methods \cite{taghibakhshi2021optimization}. 
% We also characterize AMR as a sequential decision-making problem. However, our approach differs from Yang et al.~\cite{yang2021reinforcement} and Foucart et al.~\cite{foucart2023deep} in the following ways: (1) we formulate AMR as a partially observed Markov decision process with larger observation windows and \emph{fixed}-size state and action spaces; (2) we utilize \dk{both primitive and conservative variables AND Jacobian..?}; (3) we allow multiple time steps between mesh updates.

% Need to look for more references and make sure to cite \cite{yang2022multi,gillette2022learning,foucart2023deep,sluzalec2022quasi}

% \subsection{Outline}

% Last TODO

% Insert preliminaries section about hyperbolic systems under study.


    % \begin{figure}[htbp!]
    %     \centering
    %     \adjustbox{width=0.45\linewidth,valign=b}{\input{./figs/tikz/euler_href_pareto_id}}
    %     \caption{\label{fig:euler_href_pareto_id}Mean Pareto plot of normalized cost vs. error for $h$-refinement on the Euler equations with DynAMO and the threshold policy for the two-dimensional Riemann problem over 100 \textit{in-distribution} runs using uniform random initial conditions. Contours of efficiency shown on background. Error bars represent $\pm 1$ standard deviation.}
    % \end{figure}
